Is Q-Learning Minimax Optimal? A Tight Sample Complexity Analysis

Q-learning, which seeks to learn the optimal Q-function of a Markov decision process (MDP) in a model-free fashion, lies at the heart of reinforcement learning. When it comes to the synchronous setting (such that independent samples for all state-action pairs are drawn from a generative model in each iteration), substantial progress has been made towards understanding the sample efficiency of Q-learning. Consider a $\gamma$-discounted infinite-horizon MDP with state space $\mathcal{S}$ and action space $\mathcal{A}$: to yield an entrywise $\varepsilon$-approximation of the optimal Q-function, state-of-the-art theory for Q-learning requires a sample size exceeding the order of $\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^5\varepsilon^{2}}$, which fails to match existing minimax lower bounds. This gives rise to natural questions: what is the sharp sample complexity of Q-learning? Is Q-learning provably sub-optimal? This paper addresses these questions for the synchronous setting: (1) when $|\mathcal{A}|=1$ (so that Q-learning reduces to TD learning), we prove that the sample complexity of TD learning is minimax optimal and scales as $\frac{|\mathcal{S}|}{(1-\gamma)^3\varepsilon^2}$ (up to log factor); (2) when $|\mathcal{A}|\geq 2$, we settle the sample complexity of Q-learning to be on the order of $\frac{|\mathcal{S}||\mathcal{A}|}{(1-\gamma)^4\varepsilon^2}$ (up to log factor). Our theory unveils the strict sub-optimality of Q-learning when $|\mathcal{A}|\geq 2$, and rigorizes the negative impact of over-estimation in Q-learning. Finally, we extend our analysis to accommodate asynchronous Q-learning (i.e., the case with Markovian samples), sharpening the horizon dependency of its sample complexity to be $\frac{1}{(1-\gamma)^4}$.

==> shelved/doubleQ_pieces.tex <==
Finally, we show that double Q-learning \citep{hasselt2010double} achieves the minimax sample complexity on the constructed hard MDP by mitigating the over-estimation issue. To the best of our knowledge, this is the first case study that provably demonstrates the benefits of double Q-learning over Q-learning from the sample complexity perspective.

Encouragingly, double Q-learning performs over vanilla Q-learning and can still possess minimax optimality in this case, which unveils the efficiency of double Q-learning to some extent.

==> shelved/finite-horizon-write-ups.tex <==

\subsection{Q-learning for finite-horizon MDPs} 
\label{sec:background-finite}


\paragraph{Finite-horizon MDPs.} 

We now turn attention to a finite-horizon MDP, which can be represented and described by the quintuple $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \{P_h\}_{h=1}^H, \{r_h\}_{h=1}^H, H)$. Here, $H$ represents the time horizon of the MDP. For any $1\leq h\leq H$, we let $P_h : \cS \times \cA \rightarrow \Delta(\cS)$ denote the probability transition kernel at step $h$ (i.e., $P_h(s'\mymid s,a)$ is the probability of transiting to $s'$ from $(s,a)$ at step $h$), 
and $r_h: \cS \times \cA \rightarrow [0,1]$ indicates the reward function at step $h$ (i.e., $r_h(s,a)$ is the immediate reward at step $h$ in response to $(s,a)$). As before, we assume normalized rewards so that all the $r_h(s,a)$'s reside within the range $[0,1]$. 
%In contrast to the infinite-horizon counterpart, finite-horizon MDPs do not require introducing a discount factor $\gamma$.



\paragraph{Value function and Q-function.}

Let  $\pi=\{\pi_h\}_{1\leq h\leq H}$ represent a deterministic policy such that $\pi_h(s)$ specifies the action selected at step $h$ when the current state is $s$. The value function and Q-function associated with policy $\pi$ are defined by
%
 \begin{align*}
   V^{\pi}_h (s) \coloneqq \mathbb{E} \left[ \sum_{k=h}^{H} r_k(s_k,a_k ) \,\Big|\, s_h =s \right]
\end{align*} 
%
 for all $s\in \cS$ and all $1\leq h \leq H$, and
 %
 \begin{equation*}
Q^{\pi}_h(s,a) \coloneqq \mathbb{E} \left[ \sum_{k=h}^{H} r_k(s_k,a_k ) \,\Big|\, s_h =s, a_h = a \right] 
\end{equation*} 
%
for all $(s,a)\in \cS \times \cA$  and all $1\leq h \leq H$. 
As before,  the expectations are taken over the randomness of the MDP trajectory $\{(s_k,a_k)\}_{1\leq k\leq H}$ induced by the transition kernel $\{ P_h \}_{h=1}^H$ when policy $\pi$ is adopted.
In view of the assumed bounds for the immediate rewards, it is easily seen that $0\leq V^{\pi}_h (s) \leq H$ and $0 \leq Q^{\pi}_h (s, a) \leq H$ for any $\pi$, any state-action pair $(s, a)$, and any step $h$. 
Akin to the infinite-horizon scenario, the optimal value functions $\{V_h^{\star}\}_{1\leq h\leq H}$ and optimal Q-functions $\{Q_h^{\star}\}_{1\leq h\leq H}$ are defined respectively by
%
\begin{equation*}
	V^{\star}_h(s) \coloneqq \max_{\pi} V^{\pi}_h(s)
	\qquad \text{and} \qquad
	Q^{\star}_h(s,a) \coloneqq \max_{\pi} Q^{\pi}_h(s,a)
\end{equation*}
%
for any state-action pair $(s,a)\in \cS\times \cA$ and any $1\leq h \leq H$.
% A distinguishing feature of finite-horizon MDPs is the non-stationarity of  value functions and Q-functions across $h$. 


\begin{algorithm}[t]
	\begin{algorithmic}[1] 
		\STATE\textbf{inputs:} learning rates $\{\eta_t\}$, number of iterations $T$, initial estimate $\{Q_{0, h}\}_{h=1}^H$.
%\STATE  \textbf{initialization:} $Q_0=0$. 
   \FOR{$t=1,2,\cdots,T$}
   \STATE{Set $Q_{t, H+1} = 0$.}
   \FOR{$h=H, H-1, \cdots,1$}
		\STATE{ Draw  $s_{t,h}(s,a) \sim  P_h(\cdot \mymid s,a)$ for each $(s,a)$. }
	\STATE{ Compute $Q_t$ according to \eqref{eqn:q-learning-finite} and \eqref{defn:empirical-Bellman-t-finite}.}
	\ENDFOR
\ENDFOR
   %\textbf{return:} ${Q}_{T}$. 
   \end{algorithmic} 
    \caption{Synchronous Q-learning for finite-horizon MDPs}
 \label{alg:q-finite}
\end{algorithm}

\paragraph{Q-learning.}

Assume that we have access to a generative model; in each iteration, the generative model produces an independent sample for each triple $(s,a,h)$ as follows
%
\[
	s_{t,h}(s,a) \sim P_h(\cdot \mymid s,a).
\]
%
In the $t$-th iteration,  
the synchronous Q-learning algorithm updates the Q-function estimate $Q_{t,h}: \cS \times \cA \rightarrow \mathbb{R}$ from $h = H$ to $1$ as follows:
%
\begin{equation}
\label{eqn:q-learning-finite}
	Q_{t,h}  = (1- \eta_t ) Q_{t-1,h} + \eta_t \mathcal{T}_{t,h} (Q_{t, h+1}),
	%\qquad H \geq h \geq 1. 
\end{equation}
%
where $\eta_t$ denotes the learning rate in the $t$-th iteration, and $\mathcal{T}_{t,h}$ is the empirical Bellman operator based on samples generated in the $t$-th iteration for step $h$, namely,
%
\begin{align} \label{defn:empirical-Bellman-t-finite}
	\mathcal{T}_{t,h} (Q) (s , a ) &\coloneqq 
		 r_h(s , a ) + \max_{a' \in \cA} Q(s_{t,h}, a'),   \qquad	 s_{t, h}  \equiv s_{t, h}(s,a) \sim P_h(\cdot \mymid s,a)  
\end{align}
%
for every state-action pair $(s,a) \in \cS \times \cA$. 
Here, $\mathcal{T}_{t,h}$ can also be viewed as an unbiased estimate of the Bellman operator defined for the finite-horizon case. 


In addition, the initialization $\{Q_{0, h}\}_{h=1}^H$ of the algorithm is chosen such that $0 \leq Q_{0, h}(s, a) \leq H-h+1$ for all $(s,a)$ and all $1\leq h\leq H$. Throughout this paper, the value function estimate $V_{t,h}: \cS \rightarrow \mathbb{R}$ associated with the $t$-th iterate and step $h$ is defined as
%
\begin{align}
	\label{defn:Vt-finite}
	\forall s\in \cS, ~~h\in \{1,\cdots,H\}: \qquad V_{t,h}(s) :=  \max_{a\in \cA} Q_{t,h}(s,a) .
\end{align}
%
The complete algorithm is summarized in Algorithm~\ref{alg:q-finite}.



\begin{remark}
Suppose that the probability transition kernel of the MDP is time-invariant, namely,  $P_h\equiv P$ for all $1\leq h\leq H$.
Then we only need to sample once for each $(s,a)$ --- with a total number of $|\cS||\cA|$ samples --- in each iteration $t$. This should be contrasted with the time-varying case where a total number of $|\cS||\cA|H$ samples are generated in each iteration. Both scenarios have been studied for the finite-horizon setting; see, e.g., \citet{jin2018q,sidford2018near}.
\end{remark}


\subsection{Performance guarantees: finite-horizon MDPs}
\label{sec:main-results-finite}


%At each time $t$, given the samples $\bm{P}_{t,h}$, the Q-learning
%algorithm adopts the following iterative update rule
%\begin{subequations}
%\begin{align}
%\bm{Q}_{t,h} & =(1-\eta_{t})\bm{Q}_{t-1,h}+\eta_{t}(\bm{r}_{h}+\bm{P}_{t,h}\bm{V}_{t,h+1}), \forall1\le h\le H,\\
%\bm{V}_{t,h} & =\max_{a}\bm{Q}_{t,h},\qquad\forall1\le h\le H,
%\end{align}
%\end{subequations} where $\eta_{t}>0$ denotes the learning rate
%and $\bm{Q}_{t,H+1}=\bm{0},\bm{V}_{t,H+1}=\bm{0}$.



Next, we move forward to present an analogous $\ell_{\infty}$-based sample complexity of Q-learning for finite-horizon MDPs --- the setting formulated in Section~\ref{sec:background-finite}. 
%
\begin{theorem}
\label{thm:finite-horizon-simple}
Consider an arbitrary
quantity $\delta\in(0,1)$ and $\varepsilon\in(0,1]$. Suppose that
the learning rates obey
%
\begin{subequations}
\label{eq:thm-finite-horizon-condition}
%
\begin{equation}
	\frac{1}{1+\frac{c_{1}T}{H\log^{2}T}}\le\eta_{t}\le\frac{1}{1+\frac{c_{2}t}{H\log^{2}T}},\quad0\leq t\leq T
	\label{eq:thm:finite-horizaon-eta}
\end{equation}
%
for some small enough universal constants $c_{1}\geq c_{2}>0$, and
assume that the total number of iterations $T$ obeys
%
\begin{equation}
	T\ge\frac{c_{3}H^{4}\big(\log^{3}T\big)\big(\log\frac{|\mathcal{S}||\mathcal{A}|T}{\delta}\big)}{\varepsilon^{2}}
	\label{eq:thm:finite-horizon-T}
\end{equation}
%
for some sufficiently large universal constant $c_{3}>0$. \end{subequations}
If the initialization obeys $0\leq Q_{0,h}(s,a) \leq H+1-h$ for any $(s,a)$ and any $1\le h\le H$,
then Algorithm~\ref{alg:q-finite} achieves
%
\[
	\max_{(s,a)\in \cS\times \cA, \, 1\leq h\leq H} \big| Q_{T,h}(s,a) - Q_h^{\star}(s,a) \big| \le\varepsilon
\]
%
with probability exceeding $1-\delta$. 
%
\end{theorem}
%
\begin{remark} 
	\label{remark:expected-error-finite}
	Similar to Remark \ref{remark:expected-error-inf}, an immediate consequence of Theorem~\ref{thm:finite-horizon-simple} is the following mean estimation error bound:
	%
	\[
		\mathbb{E}\Big[ \max_{s,a, h} \big| Q_{T,h}(s,a) - Q_h^{\star}(s,a) \big| \Big] \le 2\varepsilon
	\]
	%
	with the proviso that $T\ge\frac{c_{3}H^4 (\log^{3}T)\big(\log\frac{|\mathcal{S}||\mathcal{A}|H T}{\varepsilon }\big)}{\varepsilon^{2}}$.
\end{remark}
%


For the general scenario (namely, $\{P_h\}_{h=1}^H$ vary across $h$), we collect $|\cS||\cA|H$ independent samples in each iteration, 
and hence Theorem~\ref{thm:finite-horizon-simple} uncovers a sample complexity at most
%
\begin{equation}
	\widetilde{O}\Big( \frac{|\cS||\cA| H^5}{ \varepsilon^2} \Big). 
\end{equation}
%
When it comes to the special case where $P_h\equiv P$ is invariant across all $1\leq h\leq H$, our theorem continues to hold if we generate $|\cS||\cA|$ independent samples per iteration (which include one sample for each state-action pair $(s,a)$ w.r.t.~$P$), leading to a reduced sample complexity of
%
\begin{equation}
	\widetilde{O}\Big( \frac{|\cS||\cA| H^4}{ \varepsilon^2} \Big). 
\end{equation}
%
As it turns out, all this is achieved by means of the same learning rate schedules (i.e., rescaled linear or constant learning rates) as for the discounted infinite-horizon counterpart. 


